GNPassGAN: Improved Generative Adversarial Networks For Trawling Offline Password Guessing

The security of passwords depends on a thorough understanding of the strategies used by attackers. Unfortunately, real-world adversaries use pragmatic guessing tactics like dictionary attacks, which are difficult to simulate in password security research. Dictionary attacks must be carefully configured and modified to represent an actual threat. This approach, however, needs domain-specific knowledge and expertise that are difficult to duplicate. This paper reviews various deep learning-based password guessing approaches that do not require domain knowledge or assumptions about users' password structures and combinations. It also introduces GNPassGAN, a password guessing tool built on generative adversarial networks for trawling offline attacks. In comparison to the state-of-the-art PassGAN model, GNPassGAN is capable of guessing 88.03\% more passwords and generating 31.69\% fewer duplicates.

==> tables/generated.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The comparison of the data distribution in the training set, testing set and the generated passwords by PassGAN and GNPassGAN. All passwords are unique in each text file.}
\label{tab:distribution}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccc}
\hline
\textbf{Length} & \textbf{Training} & \textbf{Testing} & \textbf{PassGAN} & \textbf{GNPassGAN} \\ \hline
\textless{}=5    & 0.213\%  & 0.213\%  & 0.115\%  & 0.166\%  \\ \hline
5-8              & 47.661\% & 47.645\% & 46.079\% & 46.178\% \\ \hline
8-10             & 52.126\% & 52.142\% & 53.801\% & 53.645\% \\ \hline
\textgreater{}10 & 0        & 0        & 0.005\%  & 0.011\%  \\ \hline
\end{tabular}%
}
\end{table}

==> tables/model1.tex <==
\begin{table*}[]
  \begin{center}
    \caption{Prior deep learning models used for password guessing in the literature}
    \label{tab:models}
    \begin{tabular}{llll} 
      \hline
      \textbf{Category} & \textbf{Methods} & \textbf{Models used}& \textbf{Year}\\\hline
      Autoencoders & DPG \ & WAE, GAN & 2021 \\
      GAN & AdaMs  & GAN, HashCat & 2021 \\
      GAN & REDPACK  & IWGAN, RaGAN, HashCat, PCFG & 2020 \\
      GAN & PassGAN  & IWGAN, & 2019 \\
      Attention & Language Models   & BERT, LSTM & 2019 \\
      RNN & GENPass  & PCFG, LSTM, CNN & 2018 \\
      RNN & SPRNN  & PCFG, BiLSTM & 2018 \\
      RNN & FLA & LSTM & 2016 \\
      \hline
    \end{tabular}
  \end{center}
\end{table*}
